Jodi: Unification of Visual Generation and Understanding via Joint Modeling

Visual generation and understanding are two deeply interconnected aspects of human intelligence, yet they have been traditionally treated as separate tasks in machine learning. In this paper, we propose Jodi, a diffusion framework that unifies visual generation and understanding by jointly modeling the image domain and multiple label domains. Specifically, Jodi is built upon a linear diffusion transformer along with a role switch mechanism, which enables it to perform three particular types of tasks: (1) joint generation, where the model simultaneously generates images and multiple labels; (2) controllable generation, where images are generated conditioned on any combination of labels; and (3) image perception, where multiple labels can be predicted at once from a given image. Furthermore, we present the Joint-1.6M dataset, which contains 200,000 high-quality images collected from public sources, automatic labels for 7 visual domains, and LLM-generated captions. Extensive experiments demonstrate that Jodi excels in both generation and understanding tasks and exhibits strong extensibility to a wider range of visual domains. Code is available at https://github.com/VIPL-GENUN/Jodi.

==> tables/compare-image-quality.tex <==
\begin{tabular}{lccccccc}
  \toprule
  Method & Params. (B) & GenEval↑ & DPG-Bench↑ & ImageReward↑ & T2I-CompBench↑ & DSG↑ & HPSv2↑ \\
  \midrule
  % \multicolumn{8}{c}{Text-to-image models} \\
  % \midrule
  SDXL & 2.6 & 0.55 & 74.7 & 0.69 & 0.42 & 0.72 & 27.7 \\
  PixArt-$\Sigma$ & 0.6 & 0.54 & 80.5 & 0.87 & - & - & - \\
  PlayGroundv2.5 & 2.6 & 0.56 & 75.5 & 1.09 & - & - & - \\
  SD3-medium & 2.0 & 0.62 & 84.1 & 0.86 & - & - & - \\
  Hunyuan-DiT & 1.5 & 0.63 & 78.9 & 0.92 & - & - & - \\
  Sana-1.6B & 1.6 & 0.66 & 84.8 & 0.99 & - & - & - \\
  FLUX-schnell & 12.0 & 0.71 & 84.8 & 0.91 & - & - & - \\
  \midrule
  % \multicolumn{8}{c}{Unified models} \\
  % \midrule
  OmniGen & 3.8 & 0.70 & - & - & 0.46 & 0.66 & 27.7 \\
  OneDiffusion & 2.8 & 0.65 & - & - & 0.44 & 0.68 & 27.5 \\
  UniVG & 3.7 & 0.70 & - & - & 0.48 & 0.75 & 28.2 \\
  Ours & 1.6 & & & & & & \\
  \bottomrule
\end{tabular}
